The Moon's Many Faces: A Single Unified Transformer for Multimodal Lunar Reconstruction

Multimodal learning is an emerging research topic across multiple disciplines but has rarely been applied to planetary science. In this contribution, we propose a single, unified transformer architecture trained to learn shared representations between multiple sources like grayscale images, Digital Elevation Models (DEMs), surface normals, and albedo maps. The architecture supports flexible translation from any input modality to any target modality. Our results demonstrate that our foundation model learns physically plausible relations across these four modalities. We further identify that image-based 3D reconstruction and albedo estimation (Shape and Albedo from Shading) of lunar images can be formulated as a multimodal learning problem. Our results demonstrate the potential of multimodal learning to solve Shape and Albedo from Shading and provide a new approach for large-scale planetary 3D reconstruction. Adding more input modalities in the future will further improve the results and enable tasks such as photometric normalization and co-registration.

==> figures/tikz/results/heatmap.tex <==
\begin{tikzpicture}
    \begin{axis}[
        colormap name=viridis,
        axis line style={draw=none},
        tick style={draw=none},
        xtick={0,1,2,3},
        xticklabels={gray, dem, normals, albedo},
        xticklabel style={rotate=35, anchor=east, yshift=-0.5em},
        ytick={0,1,2,3},
        yticklabels={gray, dem, normals, albedo},
        ymin=-0.5,
        ymax=3.5,
        xmin=-0.5,
        xmax=3.5,
        width=\textwidth,
        point meta=explicit,
        nodes near coords,
        nodes near coords align={center},
        nodes near coords={%
            \pgfmathtruncatemacro{\rowy}{int(\coordindex/4)}%
            \pgfmathtruncatemacro{\colx}{int(mod(\coordindex,4))}%
            \ifnum\rowy=\colx
                --
            \else
                \pgfmathprintnumber{\pgfplotspointmeta}
            \fi
        }
    ]
        \addplot[matrix plot, mesh/rows=4, mesh/cols=4] table [x=x, y=y, meta=z] {
            x y z
            0 0 1.0 
            0 1 0.614
            0 2 0.583
            0 3 0.523
            1 0 0.492
            1 1 1.0 
            1 2 0.636
            1 3 0.375
            2 0 0.528
            2 1 0.497
            2 2 1.0 
            2 3 0.981
            3 0 0.722
            3 1 0.675 
            3 2 0.977
            3 3 1.0
        };
    \end{axis}
\end{tikzpicture}


==> sections/dataset.tex <==
\section{Dataset}
\begin{table}
	\centering
	\begin{tabular}{l c c c c}
		\hline
		\thead{Site \\ name:}	& Image ID: 	& \thead{Incidence \\ angle [\textdegree]:}	& \thead{Phase \\ angle [\textdegree]:}	& \thead{Nominal \\ Resolution [m]:} \\\hline\hline		
		Apollo 16	& M144524996	& $47.18$							& $50.98$						& $0.5$								 \\
		Apollo 17	& M168000580	& $45.13$							& $71.15$						& $0.5$								 \\
		Apollo 11	& M175124932	& $40.98$							& $39.86$						& $0.5$							     \\
		Apollo 15	& M175252641	& $49.39$							& $48.43$						& $0.5$							     \\
		Apollo 14	& M175388134	& $44.91$							& $29.33$						& $0.5$								 \\
		Apollo 12	& M175428601	& $45.16$							& $44.03$						& $0.5$								 \\\hline
	\end{tabular}
	\caption{All NAC images used in this work are constructed by stitching together both left and right side NAC images and normalizing them using ISIS3 \citep{isis3}.}
	\label{tab:data:NACImage}
\end{table}
Our dataset consists of six large narrow-angle camera (NAC) images from the Lunar Reconnaissance Orbiter (LRO) \citep{LRO1, LRO2}. Specifically, these NAC images correspond to the Apollo 11 through 17 landing sites. For the creation of our training dataset, we included images from Apollo 12, 14, 15, 16, and 17 as training samples for our tokenizers and model. By combining and slicing these large images into patches measuring $224\times 224$ pixels, with a stride of $32$, we generated a total of $1,720,540$ images. Since the tokenizers operate with a patch size of 8, this results in $784$ tokens per image. As a result, the multimodal model was trained on over $1.34$ billion tokens. For testing, we used the NAC image from the Apollo 11 landing site, which yielded $22,405$ images to evaluate the algorithm, resulting in over $17$ million tokens per modality to test with.

==> sections/shape_from_shading.tex <==
\section{Albedo Estimation and Surface Reconstruction}
\begin{figure}
    \centering
    % \includegraphics[width=0.8\linewidth]{figures/Placeholder_SfS.png}
    \input{figures/tikz/sfs/pipeline.tex}
    \caption{The SfS algorithm requires a low-resolution DEM and a grayscale image as inputs. The output high-resolution DEM, surface normals, and an albedo map are used as input for the foundation model.} 
    \label{fig:sfs-overview}
\end{figure}
To derive the Digital Elevation Models (DEMs), normal maps, and albedo maps for subsequent analysis, we utilized our Shape and Albedo from Shading (SfS) framework. This section will briefly explain the method which we previously validated for the Moon \cite{dem_grumpe2014,dem_grumpe2014_2}, Mercury \cite{tenthoff-2020}, and Mars \cite{hess-2022}. A more detailed description of the method can be found in \cite{dem_grumpe2014,dem_grumpe2014_2}.

SfS requires a reflectance model $R$ that relates the shading observed in the image $I$ to the surface shape, i.e. the DEM representing the surface. 
A DEM is a function $z(x,y)$ that assigns a height to each pixel $(x,y)$. 
The components of the surface gradient are the partial derivatives of $z$ with respect to $x$ and $y$, respectively:
\begin{equation}
    p = \frac{\partial z}{\partial x} \quad \textnormal{and} \quad q = \frac{\partial z}{\partial y}
\end{equation}
The surface normal vector $\mathbf{n}$ is defined as
\begin{equation}
    \mathbf{n} = \frac{1}{\sqrt{p^2+q^2+1}} 
    \begin{pmatrix} 
    -p \\ 
    -q \\ 
    1 
    \end{pmatrix}
\end{equation}
The surface slope angle $\alpha$ is useful for hazard assessment maps and can be derived from the surface gradient or normal vector with
\begin{equation}
    \alpha = \arctan(\sqrt{p^2+q^2}) = \arccos(n_z)   
\end{equation}

The illumination and viewing geometry is defined by the incidence angle $i$ (between $\mathbf{n}$ and $\mathbf{s}$ pointing to the Sun), the emission angle $e$ (between $\mathbf{n}$ and $\mathbf{v}$ pointing to the camera), and the phase angle $g$ (between $\mathbf{s}$ and $\mathbf{v}$). 
Instead of a simple empirical model (e.g., Lambert or Lunar-Lambert), we opt to use the more complex Hapke model \cite{hapke-2012}. 
The Hapke model is a physically based reflectance model that works well for particulate surfaces, such as the lunar regolith.
We use the Anisotropic Multiple Scattering Approximation (AMSA) \cite{hapke-2012} of the Hapke model given by 
\begin{equation}
    \begin{split}
    R_\textnormal{AMSA}(i, e, g, w) &= \frac{w}{4\pi} \frac{\mu_0}{\mu_0 + \mu} \left[ \right. p(g)B_\textnormal{SH}(g)\\ &\left. + M(\mu_0, \mu) \right]  B_\textnormal{CB}(g) S(i,e,g,\bar\theta)
    \end{split}
\end{equation}  
with $\mu_0 = \cos(i)$ and $\mu = \cos(e)$. 
The single-scattering albedo $w$ is the intrinsic reflectivity of the surface material independent of the orientation. Our SfS framework allows us to estimate the pixelwise albedo $w$ simultaneously with the DEM.
The resulting albedo map is used for the multi-modal model.
We use fixed values estimated by Warell \cite{warell-2004} for the remaining parameters of the model.
The phase function $p(g)$ is given by the Double Henyey-Greenstein function with parameters $b=0.21$ and $c=0.7$ \cite{warell-2004}. We use $B_\textnormal{S0}=3.1$ and $h_\textnormal{S}=0.11$ for the Shadow Hiding Opposition Effect $B_\textnormal{SH}$.

Every SfS algorithm is based on the minimization of the intensity error 
\begin{equation}
    E_\textnormal{I} = \frac{1}{2} \int\limits_{x}\int\limits_{y} \left(R(p,q) - I\right)^2 dx dy
\end{equation}
between the modeled reflectance image $R$ and the observed image $I$.

SfS is an ill-posed problem, because two unknowns $p$ and $q$ have to be estimated from a single pixel.
Therefore, additional regularization terms are required to obtain a solution. 
The error terms chosen for the SfS algorithm that was used in this work are described in Appendix \ref{appendix:SfS}. 
The minimization of the resulting total error is performed using an iterative relaxation approach. The update equations can be found in \cite{dem_grumpe2014}. 
Figure \ref{fig:sfs-overview} shows the input and output of the SfS algorithm.
We use the output albedo map, the DEM, and the derived surface normals as input for our foundation model.

